The Step Decay Schedule: A Near Optimal, Geometrically Decaying Learning Rate Procedure For Least Squares

Minimax optimal convergence rates for classes of stochastic convex optimization problems are well characterized, where the majority of results utilize iterate averaged stochastic gradient descent (SGD) with polynomially decaying step sizes. In contrast, SGD's final iterate behavior has received much less attention despite their widespread use in practice. Motivated by this observation, this work provides a detailed study of the following question: what rate is achievable using the final iterate of SGD for the streaming least squares regression problem with and without strong convexity? First, this work shows that even if the time horizon T (i.e. the number of iterations SGD is run for) is known in advance, SGD's final iterate behavior with any polynomially decaying learning rate scheme is highly sub-optimal compared to the minimax rate (by a condition number factor in the strongly convex case and a factor of $\sqrt{T}$ in the non-strongly convex case). In contrast, this paper shows that Step Decay schedules, which cut the learning rate by a constant factor every constant number of epochs (i.e., the learning rate decays geometrically) offers significant improvements over any polynomially decaying step sizes. In particular, the final iterate behavior with a step decay schedule is off the minimax rate by only $log$ factors (in the condition number for strongly convex case, and in T for the non-strongly convex case). Finally, in stark contrast to the known horizon case, this paper shows that the anytime (i.e. the limiting) behavior of SGD's final iterate is poor (in that it queries iterates with highly sub-optimal function value infinitely often, i.e. in a limsup sense) irrespective of the stepsizes employed. These results demonstrate the subtlety in establishing optimal learning rate schemes (for the final iterate) for stochastic gradient procedures in fixed time horizon settings.

==> tex/algos.tex <==
\begin{figure}%\vspace*{-5pt}
	\begin{minipage}{.55\textwidth}
		\begin{algorithm}[H]
			\caption{\osgd: Stochastic Gradient Descent with oscillating learning rates}
			\label{alg:osgd}
			\begin{algorithmic}[1]
				\REQUIRE Initial guess $\w_0$, smoothness $L$, strong convexity parameter $\mu$, total number of steps $N$.
				\STATE	$\kappa=L/\mu$.
				%\STATE $t \leftarrow 0$
				\FOR{$t=1,\cdots,\lceil\log(\kappa)\rceil$}
				\STATE	\begin{align*}
				\eta^{(t)}_l = \begin{cases}
				1/L,\ \quad\quad\quad\quad\quad 1\leq l\leq\lceil\kappa/2^{t-1}\rceil. \\
				\frac{1}{\mu\cdot \left(\lceil N/\log{(\kappa)}\rceil- \lceil\kappa/2^{t-1}\rceil\right)},\\\quad\quad\quad \lceil\kappa/2^{t-1}\rceil< l\leq\lceil N/\log{(\kappa)}\rceil .
				\end{cases}
				\end{align*}
				\STATE $\w_t\leftarrow$\sgd$(\w_{t-1},\eta^{(t)}_{1:\lfloor N/\lceil\log(\kappa)\rceil\rfloor})$/*Algorithm~\ref{alg:sgd}*/
				\ENDFOR
				\RETURN $\w_{\text{op}}\leftarrow\w_{\lceil\log(\kappa)\rceil}$ /*Return the last iterate*/
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}\hspace*{5pt}
	\begin{minipage}{.45\textwidth}
		\begin{algorithm}[H]
			\caption{\sgd: Stochastic Gradient Descent with a time-varying learning rates}
			\label{alg:sgd}
			\begin{algorithmic}[1]
				\REQUIRE Initial guess $\w_0$, learning rate $\{\eta_t\}_{t=1}^T$
				\FOR{$t=1,\cdots,T$}
				\STATE	$\w_t = \w_{t-1}-\eta_t\cdot\sgflin{\w_{t-1},\xi_t}$ \ENDFOR
				\RETURN $\w_t$ \hfill /*Return the last iterate*/
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
\end{figure}

We present Algorithm~\ref{alg:osgd}, which is an epoch based algorithm which runs for a total of $\lceil\log{(\kappa)}\rceil$ epochs. Algorithm~\ref{alg:osgd} requires the knowledge of the smoothness parameter $L$ (akin to standard SGD), total number of steps $N\left(\gtrsim\kappa\log(\kappa) \right)$, the strong convexity parameter $\mu$ (which is considered available even in the standard analyses of SGD for strongly convex objectives). %In epoch $t$, runs with a learning rate of $1/L$ for a total of $\lceil\kappa/2^{t-1}\rceil$ steps, thus making progress on all eigen directions $\lambda\in[\lammaxH/2^{t-1},\lammaxH]$. However, the error does not decay on all eigenvalues $\lambda\in[\mu,\lammaxH/2^{t-1})$.

We will now present the guarantee of Algorithm~\ref{alg:osgd}.
\begin{theorem}
	\label{thm:osgd}
	Running Algorithm~\ref{alg:osgd} for a total of $N\gtrsim\kappa\log(\kappa)$ steps starting at an iterate $\w_0$, a smoothness parameter $L$, strong convexity $\mu$ yields a output $\w_{\text{op}}$ that satisfies the following gradient norm guarantee:
	\begin{align*}
		\E{\|\nabla \flin(\w_{\text{op}})\|^2} \lesssim \log{(\kappa)}\frac{\Tr{(\V)}}{N}.
	\end{align*}
\end{theorem}

The proof of theorem~\ref{thm:osgd} is found in the appendix. Note that the result of Theorem~\ref{thm:osgd} is in stark contrast to the behavior of standard SGD for the gradient norm, which we present below.

==> tex/setup.tex <==
%\praneeth{Go over. Connect to linear regression.}

\textbf{Notation}: We represent scalars with normal font $a, b, L$ etc., vectors with boldface lowercase characters $\a,\bb$ etc. and matrices with boldface uppercase characters $\A,\B$ etc. We represent positive semidefinite (PSD) ordering between two matrices using $\succeq$. The symbol $\gtrsim$ represents that the direction of inequality holds for some universal constant. 

Our theoretical results focus on the following additive noise stochastic quadratic optimization problem.
We present the setup and associated notation in this section. We wish to solve:
\begin{align}\label{eq:objectiveFn}
\min_{\w \in \R^d} f(\w) \, \textrm{ where } f(\w) \eqdef \frac{1}{2} \w^{\top} \Cov \w - \w^\top \bb \,
\end{align}
for some positive semidefinite matrix $\Cov$ and vector $\bb$. Note that the Hessian of $f$ is $\nabla^2 f = \Cov$.
%\footnote{Any linear least squares $\frac{1}{2n} \sum_{i=1}^{n} \left(\x_i^\top \w - y_i\right)^2$ can be written as above with $\Cov \defeq \frac{1}{n}\sum_i\x_i \x_i^{\top}$ and $\b \defeq \frac{1}{n} \sum_iy_i \x_i$.}
We denote by
\begin{align*}
\mu \eqdef \lambda_{\textrm{min}}\left(\Cov\right), \quad
L \eqdef \lambda_{\textrm{max}}\left(\Cov\right), \mbox{  and },
\kappa \eqdef \frac{L}{\mu}
\end{align*}
the smallest eigenvalue, largest eigenvalue and condition number of $\Cov$ respectively. $\mu > 0$ in the strongly convex case but not necessarily so in the non-strongly convex case (in section~\ref{sec:comparison}, the non-strongly convex case is referred to as the ``smooth'' case). We consider stochastic gradient oracle with the additive noise assumption, which corresponds to the first setting studied in stochastic approximation~\citep{RobbinsM51,PolyakJ92,duflo2013random}.
More concretely, we assume access to stochastic gradients $\widehat{\nabla} f(\w)$, which satisfy the following assumptions:
\begin{align}
\widehat{\nabla} f(\w) = \nabla f(\w) + \e,\quad \E{\e}=0 \, \textrm{ and } \E{\e \e^{\top}} \preceq \sigma^2 \Cov. \label{eq:noise}
\end{align}
The above assumptions (which are the same as $\mathcal{A}4$ and $\mathcal{A}5$ in~\cite{DieuleveutFB16}) bear a close relationship to ones employed in analyzing stochastic linear regression~\footnote{Suppose $y=\langle w^*,x\rangle+\epsilon$ with $\epsilon\sim\mathcal{N}(0,\sigma^2)$. For optimizing $F(w)=\E{(y-\langle w,x\rangle)^2}$, the stochastic gradient over a single example $(x,y)$ has the following covariance at $w^*$, i.e.,  $\E{\widehat{\nabla}F(\w^*)\widehat{\nabla}F(\w^*)^\top}=\E{\epsilon^2 xx^\top}\preceq\sigma^2\Cov$.\label{slr-connection}}. Refer to~\cite{DieuleveutFB16} for a discussion.%\textbf{Assumption on the noise covariance matrix}: Related to linear least squares regression.

%\footnote{While this might seem very special, this is indeed a fairly natural scenario. For instance, in stochastic linear regression with independent additive noise, i.e., $y_t = \x_t^{\top} \ws + \epsilon_t$ where $\epsilon_t$ is a random variable independent of $\x_t$ and $\E{\epsilon_t}=0$ and $\E{\epsilon_t^2}=\sigma^2$, the noise in the gradient has this property. On the other hand, the results in this paper can also be generalized to the setting where $\E{\e\e^{\top}}=\V$ for some arbitrary matrix $\V$. However, error covariance of $\sigma^2 \Cov$ significantly simplifies exposition.}
%Note that our upper bounds function with the above bound on the covariance of the error $\e$, whilst for the lower bounds in this paper (where we require a specific problem instance), we function with the above assumption, but with an equality.
\noindent
Given an initial point $\w_0$ and step size sequence $\eta_t$, the SGD algorithm proceeds with the update
\begin{align*}
\w_t = \w_{t-1} - \eta_t \widehat{\nabla} f(\w_{t-1}) = \w_{t-1} - \eta_t \left({\nabla} f(\w_{t-1}) + \e_t\right),
\end{align*}
where $\e_t$ are independent for different $t$ and satisfy~\eqref{eq:noise}.

Let $\ws \defeq \argmin_{\w \in \Rd} f(\w)$. The suboptimality of a point $\w$ is given by $f(\w)-f(\ws)$. It is well known that given $t$ accesses to the stochastic gradient oracle above, any algorithm that uses these stochastic gradients and outputs $\widehat{\w}_t$ has suboptimality that is lower bounded by $\frac{\sigma^2 d}{t}$. More concretely, we have that~\citep{van2000asymptotic}
\[
\lim_{t\rightarrow \infty} \frac{\E{f(\widehat{\w}_t)}-f(\ws)}{\sigma^2 d /t} \geq 1 \, .
\] There exists schemes that achieve this rate of $\left(1+o(1)\right) \frac{\sigma^2 d}{t}$ e.g., constant step size SGD with averaging~\citep{PolyakJ92}. This rate of $\sigma^2 d /t$ is called the statistical minimax rate.
%The goal in standard Machine Learning/Optimization is to approximately compute:
%\begin{align*}
%	\ws\in\arg\min_{\w\in\Rd}f(\w)\defeq \frac{1}{n}\sum_{i=1}^n f(\w;(\x_i,y_i)),
%\end{align*}
%where, $f(\cdot)$ is a desired objective function (e.g. square loss/softmax loss) to be optimized, $\ST=\{\x_i,y_i\}_{i=1}^n$ is the dataset with $\x_i\in\Rd$ being the input, $y_i\in\R$ being the target and $\w$ is the set of model parameters. A specific focus of this paper is the square loss objective:
%\begin{align}
%	\label{eq:linObj}
%	\flin(\w) = \frac{1}{n}\sum_{i=1}^n \tfrac{1}{2}(y_i-\iprod{\w}{\x_i})^2,
%\end{align}
%Note that the Hessian $\Cov$ of the objective function $\flin(\cdot)$ is constant at all the points in the domain, and is represented below:
%\begin{align}
%	\label{eq:linHess}
%	\Cov\defeq\nabla^2 \flin(\w) = \frac{1}{n}\sum_i \x_i\x_i\T.
%\end{align}
%The smoothness parameter $L$ doubles up as the largest eigenvalue of the hessian H, i.e., $L\defeq\lammaxH$. With this in place, the condition number of the problem $\kappa\defeq L/\mu$. Now, in order to minimize $\flin(\cdot)$, we are provided access to a \sfo~(\sfoa), which when queried at a specific iterate $\w$, returns a stochastic estimate $\sgflin{\w;\xi}$ of the true gradient $\gflin{\w}$ at $\w$. Note that $\xi$ is a random variable (that is independent of $\w$ and is) drawn from some unknown distribution $\DT$ whose properties we will make precise through our assumptions below. Before we go over the assumptions, the underlying algorithm that we will consider closely is Stochastic Gradient Descent (\sgd), wherein, we employ the stochastic gradient returned by the \sfoa~ to move $\w$ to the next iterate $\w^{+}$, i.e.,
%%In order to minimize the objective function $f$ (or $\flin$), we are given access to a \sfo~(\sfoa), which when queried at a specific iterate $\w$, returns a stochastic estimate $\sgf{\w;\xi}$ (or, $\sgflin{\w;\xi}$) of the true gradient $\gf{\w}$ (or $\gflin{\w}$) at $\w$. Note that $\xi$ is a random variable (that is independent of $\w$ and is) drawn from some underlying distribution $\DT$ whose properties we will make precise through our assumptions below. Before we go over the assumptions, the underlying algorithm that we will consider closely is Stochastic Gradient Descent (\sgd), wherein, we employ the stochastic gradient returned by the \sfoa~ to move us to the next iterate $\w^{+}$, i.e.,
%\begin{align*}
%\w^+ \leftarrow \w - \gamma_{\w}\cdot \sgflin{\w;\xi},
%\end{align*}
%where, $\eta_{\w}>0$ is a learning rate/step size.
%\paragraph{Assumptions:}
%We make the following assumptions in the context of the objective function $\flin(\cdot)$ and the corresponding stochastic first order oracle:
%\begin{enumerate}%[label=$\mathbf{(\mcA\arabic*)}$]
%	\item \label{asmp:scvx} {\bf Strong Convexity:} We assume that the objective function $\flin(\cdot)$ (equation~\ref{eq:linObj}) is strongly convex, or equivalently, the Hessian $\Cov$ is positive definite, i.e. $\Cov\succ 0$. This implies that the minimizer of equation~\ref{eq:linObj} (i.e. $\ws$) is unique and the smallest eigenvalue $\mu=\lamminH>0$.
%	\item \label{asmp:unbiasedness} {\bf Unbiased estimates:} The stochastic gradients returned by the \sfoa~ are unbiased, i.e., 
%	\begin{align*}
%	\Eover{\xi\sim\DT}{\sgflin{\w;\xi}|\w}=\gflin{\w}.
%	\end{align*}
%	\item \label{asmp:boundedVariance} {\bf Bounded Covariance of Stochastic Gradients:} The covariance matrix of the Stochastic Gradients is strictly bounded, i.e., 
%	\begin{align}
%	\label{eq:linVarBound}
%	\Eover{\xi\sim\DT}{(\sgflin{\w;\xi}-\gflin{\w})(\sgflin{\w;\xi}-\gflin{\w})\T | \w} \preceq \V.
%	\end{align}
%\end{enumerate}
%
%Assumption~\ref{asmp:unbiasedness},~\ref{asmp:boundedVariance} indicates that $\sgflin{\w;\xi}$ can be written in the following manner:
%\begin{align}
%\label{eq:sgExp}
%\sgflin{\w;\xi} = \gflin{\w} + \nv = \Cov(\w-\ws)+\nv, \text{ with, } \E{\nv|\w} = \zo, \E{\nv\nv\T|\w} \preceq \V.
%\end{align}
